Towards Terabit LiFi Networking

Light Fidelity (Li-Fi) is a networked version of optical wireless communication (OWC), which is a strong candidate to fulfill the unprecedented increase in user-traffic expected in the near future. In OWC, a high number of optical access points (APs) is usually deployed on the ceiling of an indoor environment to serve multiple users with different demands. Despite the high data rates of OWC networks, due to the use of the optical band for data transmission, they cannot replace current radio frequency (RF) wireless networks where OWC has several issues including the small converge area of an optical AP, the lack of uplink transmission and high blockage probabilities. However, OWC has the potential to support the requirements in the next generation (6G) of wireless communications. In this context, heterogeneous optical/RF networks can be considered to overcome the limitations of OWC and RF systems, while providing a high quality of service in terms of achievable data rates and coverage. In this work, infrared lasers, vertical-cavity surface-emitting(VCSEL) lasers, are used as the key elements of optical APs for serving multiple users. Then, transmission schemes such as zero forcing (ZF) and blind interference alignment (BIA) are introduced to manage multi-user interference and maximize the sum rate of users. Moreover, a WiFi system is considered to provide uplink transmission and serve users that experience a low signal to noise ratio (SNR) from the optical system. To use the resources of the heterogeneous optical/RF network efficiently, we derive a utility-based objective function that aims to maximize the overall sum rate of the network.

==> Source files/main.tex <==

\input{./text.tex} %Preamble
\begin{document}
\frontmatter
\input{./apalike.sty}
\input{./article.cls}
\input{./SCITEPRESS.sty}
\input{./figures/fig.pdf}
\maketitle
\tableofcontents{}
\mainmatter
    %...\input various %
    %...\chapters ...  %     
\end{document}


==> main.tex <==

\input{./text.tex} %Preamble
\begin{document}
\frontmatter
\input{./apalike.sty}
\input{./article.cls}
\input{./SCITEPRESS.sty}
\input{./figures/fig.pdf}
\maketitle
\tableofcontents{}
\mainmatter
    %...\input various %
    %...\chapters ...  %     
\end{document}

